Haptic Rendering of Cultural Heritage Objects at Different Scales

In this work, we address the issue of a virtual representation of objects of cultural heritage for haptic interaction. Our main focus is to provide haptic access to artistic objects of any physical scale to the differently-abled people. This is a low-cost system and, in conjunction with a stereoscopic visual display, gives a better immersive experience even to the sighted persons. To achieve this, we propose a simple multilevel, proxy-based hapto-visual rendering technique for point cloud data, which includes the much-desired scalability feature which enables the users to change the scale of the objects adaptively during the haptic interaction. For the proposed haptic rendering technique, the proxy updation loop runs at a rate 100 times faster than the required haptic updation frequency of 1KHz. We observe that this functionality augments very well with the realism of the experience.

==> abstract.tex <==
\begin{abstract}
In this work, we address the issue of virtual representation of objects of cultural heritage. Our main 
focus is to provide a haptic access of artistic objects of any physical scale to the differently abled
people. This is a low-cost system and in conjunction with a stereoscopic visual display gives a better immersive experience even to the sighted persons. 
To achieve this, we propose a simple multilevel, proxy-based hapto-visual rendering technique. 
We also propose some additional features like scalability which enable the users to change the scale 
of the objects adaptively during the haptic interaction. The haptic rendering technique proposed in this
paper is a proxy based one with proxy updation loop running at a rate of more than 100 times faster 
than the required haptic updation frequency of 1KHz. We observe that this functionality augments very well 
to the realism of the experience. 
  

\end{abstract}

\begin{keywords}

Haptic rendering, HIP, proxy-based rendering, voxel-based rendering, image-pyramid, Gaussian kernel, stereoscopic display.

\end{keywords}
